TriggerNER: Learning with Entity Triggers as Explanations for Named Entity Recognition

Training neural models for named entity recognition (NER) in a new domain often requires additional human annotations (e.g., tens of thousands of labeled instances) that are usually expensive and time-consuming to collect. Thus, a crucial research question is how to obtain supervision in a cost-effective way. In this paper, we introduce "entity triggers," an effective proxy of human explanations for facilitating label-efficient learning of NER models. An entity trigger is defined as a group of words in a sentence that helps to explain why humans would recognize an entity in the sentence. We crowd-sourced 14k entity triggers for two well-studied NER datasets. Our proposed model, Trigger Matching Network, jointly learns trigger representations and soft matching module with self-attention such that can generalize to unseen sentences easily for tagging. Our framework is significantly more cost-effective than the traditional neural NER frameworks. Experiments show that using only 20% of the trigger-annotated sentences results in a comparable performance as using 70% of conventional annotated sentences.

==> table0-main_table.tex <==
\begin{table}[tb!]
\caption{Performance comparison on temporal link prediction (average metrics in \% over 5 runs) on three event-based TKG datasets with filtered setting. \method achieves the best results. 
Results with raw setting are in the supplementary material.
}
\label{result:filtered}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccccccccc}
\cmidrule[1pt](){2-14}
    \multicolumn{2}{c}{\multirow{2}{*}{\vspace{-2.2mm}\textbf{Method}}} & \multicolumn{4}{c}{\textbf{ICEWS18 - filtered}} & \multicolumn{4}{c}{\textbf{GDELT - filtered}} & \multicolumn{4}{c}{\textbf{ICEWS14 - filtered}} \\ \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
       & & MRR  &H@1  &H@3  &    H@10        & MRR     &H@1&     H@3        & H@10 & MRR     &H@1&     H@3        & H@10      \\ 
\cmidrule{2-14}
\multirow{6}{*}{\rotatebox{90}{\hspace*{-6pt}Static}} 
&TransE & 17.56 & 2.48&	26.95&	43.87 & 16.05&	0.00&26.10&	42.29 & 18.65&	1.21&	31.34&	47.07   \\
&DistMult   &22.16 & 12.13&	26.00&	42.18  &	 18.71&	11.59&20.05&	32.55& 19.06&	10.09&	22.00&	36.41 \\
&ComplEx    &30.09 & 21.88&	34.15&	45.96 &  22.77&	15.77&24.05&	36.33  & 24.47 & 16.13&	27.49&	41.09  \\
&R-GCN  &23.19& 16.36&	25.34&	36.48 & 23.31&	17.24&24.94&	34.36 & 26.31 &18.23&	30.43&	45.34\\
&ConvE  &36.67& 28.51&	39.80&	50.69 &  35.99&	27.05 & 39.32 & 49.44& 40.73 & 33.20&	43.92&	54.35\\
&RotatE    & 23.10&	14.33&	27.61&	38.72 & 22.33&	16.68&	23.89&	32.29& 29.56&	22.14&	32.92&	42.68\\
% &MLP    & 41.10&	33.98&	43.86&	54.83 & 40.35&	33.22&	43.09&	53.47& 43.05&	35.14&	46.70&	57.63\\
\cmidrule{2-14}
\multirow{13}{*}{\rotatebox{90}{\hspace*{-6pt}Temporal}}
&HyTE   &7.31& 3.10 & 	7.50& 14.95 & 6.37&	0.00&6.72&	18.63& 11.48&	5.64&	13.04&	22.51\\ 
&TTransE    &8.36& 1.94&	8.71&	21.93 & 5.52&	0.47&	5.01&	15.27& 6.35&	1.23&	5.80&	16.65 \\
% &TA-TransE  &12.85 & 0.00 &	19.04&	37.53& 16.62&	0.00&27.65&	42.53  & 17.36&	0&	29.50&	47.02\\ 
&TA-DistMult    &28.53& 20.30&	31.57&	44.96  & 29.35& 22.11	&31.56&	41.39& 20.78&	13.43&	22.80&	35.26\\ 
&Know-Evolve*   & 3.27& 3.23 &	3.23&	3.26 & 2.43&	2.33 &2.35&	2.41  & 1.42&	1.35&	1.37&	1.43\\ 
&Know-Evolve+MLP    & 9.29&	5.11&	9.62&	17.18 & 22.78&	15.40&	25.49&	35.41& 22.89&	14.31&	26.68&	38.57\\ 
&DyRep+MLP  & 9.86&	5.14&	10.66&	18.66 & 23.94&	15.57&	27.88&	36.58& 24.61&	15.88&	28.87&	39.34\\ 
&R-GCRN+MLP & 35.12&	27.19&	38.26&	50.49 &37.29&	29.00&	41.08&	51.88& 36.77&	28.63&	40.15&	52.33\\ 
\cmidrule{2-14}
&\method w/o multi-step & 40.05&	33.32&	42.60&	52.92 & 38.72&	30.57&	42.52&	52.78& 42.72&	35.42&	46.06&	56.15\\ 
&\method w/o agg. & 33.46&	26.64&	35.98&	46.62 & 38.10&	29.34&	41.26&	51.61& 42.23&	34.73&	45.61&	56.07\\ 
&\method w. mean agg. & 40.70&	34.24&	43.27&	53.65 & 38.35&	29.92&	42.13&	52.52& 43.79&	36.21&	47.34&	57.47\\
&\method w. attn agg. & 40.96 &	 34.57&	44.08 & 54.32&	38.54& 29.65&	42.25& 52.85 &	43.94&	37.01&  47.85 & 57.91	\\
&\method & \textbf{42.93}&	\textbf{36.19}&	\textbf{45.47}&	\textbf{55.80} & \textbf{40.12} &	\textbf{32.43} &	\textbf{43.40}&	\textbf{53.80}& \textbf{45.71}&	\textbf{38.42}&	\textbf{49.06}&	\textbf{59.12}	\\
\cmidrule{2-14}
&\method w. GT $(\bs, \br)$ & 44.33&	37.61&	46.83&	57.27 & 41.80&	33.54&	45.71&	56.03& 46.74&	39.41&	50.10&	60.19	\\ 
% \method (Gold)  & xxx & xxx & xxx &	xxx & xxx & xxx  & xxx	&\\
%\bottomrule
\cmidrule[1pt](){2-14}
\end{tabular}}
% \vspace{-0.2cm}
\end{table}

==> table1-multi-column.tex <==
\begin{table}[t]
	\centering
	\scalebox{0.63
	}{
		\begin{tabular}{@{}lccccccccc@{}}
			\toprule   
			&      
			\multicolumn{2}{c}{Easy Mode}  &  
			\multicolumn{2}{c}{Hard Mode}  &  
			\\
			
			\textbf{Model}&     
			\multicolumn{1}{c}{IHdev.(\%)}  &    \multicolumn{1}{c}{IHtest.(\%)}  &
			\multicolumn{1}{c}{IHdev.(\%)}  &    \multicolumn{1}{c}{IHtest.(\%)}   
			\\ 
			
			Random guess &   33.3& 33.3& 20.0& 20.0\\
			\midrule \midrule 
			\textsc{BLSTMs} &   80.15 & 78.01& 34.79 &32.12  \\
			\textsc{+ KV-MN} &  81.71 & 79.63& 35.70 & 33.43\\  
			 
			\textsc{+ CSPT} &   81.79 & 80.01 & 35.31 & 33.61  \\
			\textsc{+ TextGraphCat} & 82.68  & 81.03 & 34.72 & 33.15  \\   
			\textsc{+ TripleString} &   79.11 & 76.02 & 33.19 & 31.02 \\
			\textsc{+ \textbf{KagNet}} &  83.26 & \textbf{82.15} & 36.38 & \textbf{34.57}  \\  
			\midrule\midrule
			Human Performance &  - & \textit{99.5}& - & \textit{88.9}  \\
			\bottomrule
		\end{tabular}
	} 
	\caption{Comparisons with knowledge-aware baseline methods using the in-house split (both easy and hard mode) on top of BLSTM as the sentence encoder. }
	\label{tab:knowres}
\end{table}

==> table_4-ablation.tex <==
\begin{table*}[hbt!]
\small
\begin{center}
\begin{tabular}{ c | c c c c | c c c c }
\toprule
Setting & \multicolumn{4}{c|}{Generated Test Set} & \multicolumn{4}{c}{Manual Matching Test Set}\\
 & Accuracy & Micro F\textsubscript{1} & $<$next$>$ F\textsubscript{1} & $<$if$>$ F\textsubscript{1} & Accuracy & Micro F\textsubscript{1} & $<$next$>$ F\textsubscript{1} & $<$if$>$ F\textsubscript{1}\\
\midrule
BERT & 81.6 \textpm 1.0 & 70.1 \textpm 1.7 & 67.9 \textpm 3.2 & 73.4 \textpm 2.2 & 77.2 \textpm 2.7 & 62.2 \textpm 6.1 & 57.6 \textpm 6.4
& 72.4 \textpm 10.0\\
HBMP & 76.0 & 67.4 & - & - & 72.0 & 63.3 & - & - \\
PCNN & 58 & 40 & - & - & 56 & 43 & - & - \\
\midrule
C. Attn. & 82.5 \textpm 1.5 & 72.2 \textpm 2.6 & \textbf{70.9 \textpm 1.8} & 74.7 \textpm 4.4 & 81.2 \textpm 4.7 & 72.7 \textpm 7.5 & 68.7 \textpm
9.1 & \textbf{83.3 \textpm 5.5}\\
C. Emb. & \textbf{82.8 \textpm 1.4} & 72.7 \textpm 1.9 & 70.7 \textpm 2.8 & 76.3 \textpm 2.5 & 78.8 \textpm 8.5 & 67.4 \textpm 8.1 & 66.2 \textpm 9.2 & 67.5 \textpm 19.4\\
Mask\textsubscript{AVG} & 80.5 \textpm 2.7 & 69.0 \textpm 5.7 & 63.6 \textpm 7.1 & \textbf{77.0 \textpm 4.8} & 80.4 \textpm 7.1 & 73.4 \textpm 7.9 & 71.8 \textpm 9.4 & 79.2 \textpm 14.5\\
Mask\textsubscript{MAX} & 82.3 \textpm 1.4 & \textbf{72.6 \textpm 3.0} & 70.7 \textpm 3.2 & 76.1 \textpm 3.1 & \textbf{87.6 \textpm 1.5} & \textbf{81.4 \textpm 2.4} & \textbf{80.8 \textpm 1.9} & 83.3 \textpm 6.8\\
\bottomrule
\end{tabular}
\caption{\textbf{Performance of span-pair RE models,} with sampling portion $4 : 2 : 1$ and $K=2$. Evaluated on generated test set and manual matching test set.}
\label{tab:re}
\end{center}
\end{table*}
